Settling the Communication Complexity for Distributed Offline Reinforcement Learning

We study a novel setting in offline reinforcement learning (RL) where a number of distributed machines jointly cooperate to solve the problem but only one single round of communication is allowed and there is a budget constraint on the total number of information (in terms of bits) that each machine can send out. For value function prediction in contextual bandits, and both episodic and non-episodic MDPs, we establish information-theoretic lower bounds on the minimax risk for distributed statistical estimators; this reveals the minimum amount of communication required by any offline RL algorithms. Specifically, for contextual bandits, we show that the number of bits must scale at least as $\Omega(AC)$ to match the centralised minimax optimal rate, where $A$ is the number of actions and $C$ is the context dimension; meanwhile, we reach similar results in the MDP settings. Furthermore, we develop learning algorithms based on least-squares estimates and Monte-Carlo return estimates and provide a sharp analysis showing that they can achieve optimal risk up to logarithmic factors. Additionally, we also show that temporal difference is unable to efficiently utilise information from all available devices under the single-round communication setting due to the initial bias of this method. To our best knowledge, this paper presents the first minimax lower bounds for distributed offline RL problems.

==> unused.tex <==
\section{Context/Feature vectors construction}
We will now describe the method we use to construct feature/context vectors in the instances of problems we use to derive the lower bounds. To preserve generality, we will denote by $N$ the number of feature/context vectors. Hence in the contextual bandit case $N = n$ and in full MDP case $N =  S$. In both cases the dimensionality of context/feature vectors is $ C$. For simplicity we assume $N$ is a multiple of $ C$, i.e. there exists an integer $k$ such that $ C = k N$. We start by choosing $ C$ orthogonal vectors in $ C$ dimensional space, each with norm 1, which we denote $f_1,\dots,f_{ C}$. This must always be possible, which follows from Gram-Schmidt procedure. We assign the vector for $i$th state/sample as $\vc_i = \sqrt{\lambda_{\textrm{min}}}f_{i\%k + 1}$, where $\%$ denotes the modulo operator. We now investigate how the $X^TX$ matrix looks like:
\begin{equation*}
    X^TX = 
    \lambda_{\textrm{min}}
    \begin{bmatrix}
    f_1 & \dots & f_{ C}  \dots f_1 & \dots & f_{ C} 
    \end{bmatrix}
    \begin{bmatrix}
    f_1 \\
    \dots \\
    f_{ C} \\
    \dots \\
    f_1 \\
    \dots \\
    f_{ C} 
    \end{bmatrix} =
    \lambda_{\textrm{min}}
    \begin{bmatrix}
    k & 0 & \dots & 0 \\
    0 & k & \dots & 0 \\
    \dots & \dots & \dots & \dots \\
    0 & 0 & \dots & k
    \end{bmatrix}
\end{equation*}
Where the result follows since we effectively have $k$ orthogonal matrices stacked together. We thus get that $X^TX$ is a diagonal matrix. Eigenvalues of a diagonal matrix are simply its entries, hence we see that the smallest eigenvalue of $X^TX$ is equal to $\lambda_{\textrm{min}}k = \lambda_{\textrm{min}}\frac{N}{ C}$ and that the norm of each vector is $\lambda_{\textrm{min}} \le 1$. 

\section{Unused results}
\subsection{Different number of samples}
Assume $i$th centre receives at most $n_{i}$ samples for each arm, where the $k$th sample from $j$th arm is denoted as $X_{k,j}^{i}$. Denote by $A_{k}^{i}$ set of actions for which the $i$th centre has at least $k$ samples. The reward for each arm comes from a normal distribution with unknown mean $\mu_{j}$ and variance $\sigma^{2}$.
\begin{theorem} (Not very sharp lower bound)
In a distributed offline MAB problem with $ A$ actions under the assumptions above, given $m$ processing centres each with $n$ samples (from any arm), with total communication budget $B$, for any independent communication protocol, the minimax risk $M$ is lower bounded as follows:
\begin{equation*}
    M \ge \Omega \Bigg ( \frac{\sigma^{2} A^{2}}{mn} \Bigg)
\end{equation*}
\end{theorem}
\begin{proof}
Choose $V_{j} \in \{-1,1\}$ uniformly and sample $X_{j}^{i} \sim N(\delta V,\sigma^{2})$. We will bound the mutual information $I(V, Y_{1:m})$ as follows:
\begin{equation}
\label{eq:simple_info_bound}
    I(V,Y_{1:m}) \le \sum_{i=1}^{m}I(V,Y_{i}) \le \sum_{i=1}^{m} I(V,X_{i}) \le \sum_{i=1}^{m} \sum_{k=1}^{n_{i}} \sum_{j \in A_{k}^{i}} I(V, X_{k,j}^{i}) \le \sum_{i=1}^{m} \sum_{k=1}^{n_{i}} \sum_{j \in A_{k}^{i}} \frac{\delta^{2}}{\sigma^{2}}
\end{equation}
Where the first inequality follows from tensorisation of information ((Lemma \ref{lemma:tenorisationinfo})), the second follows from the data-processing inequality, the third follows from the independence of $X_{k,j}$ (\cite{NIPS2013Yuchen}-page 16) and the final inequality is from a bound on Gaussian information (\cite{NIPS2013Yuchen} - page 16). Since the total number of samples each centre has is $n$, the triple sum is equal to $\frac{mn\delta^{2}}{\sigma^{2}}$. Using the method from Appendix \ref{appendix:minimaxlb}, we get that:
\begin{equation*}
    M \ge \delta^{2} \Big (\floor{\frac{ A}{6}} + 1 \Big ) \Bigg ( 1 - \frac{\frac{mn\delta^{2}}{\sigma^{2}} + \log2}{\frac{ A}{6}} \Bigg )
\end{equation*}
We want to set $\delta$ such that $1 > \frac{\frac{mn\delta^{2}}{\sigma^{2}} + \log2}{\frac{ A}{6}}$ (otherwise the bound is not very useful), we can see that this happens when $\delta^{2} < \frac{\sigma^{2}}{mn}(\frac{ A}{6} - \log2)$, hence we can set $\delta^{2} = c\frac{\sigma^{2}}{mn}(\frac{ A}{6} - \log2)$ for some universal constant $c > 0$. This gives:
\begin{equation*}
    M \ge c\frac{\sigma^{2}}{mn}(\frac{ A}{6} - \log2) \Big (\floor{\frac{ A}{6}} + 1 \Big ) = \Omega \bigg (\frac{\sigma^{2} A^{2}}{mn} \bigg )
\end{equation*}
\end{proof}
\begin{theorem} (Sharper Lower Bound) \label{th:sharper_lb_mab}
In a distributed offline MAB problem with $ A > 12$ actions under the assumptions above, given $m$ processing centres each with $n$ samples (from any arm), with total communication budget $B \ge 1$, for any independent communication protocol, the minimax risk $M$ is lower bounded as follows:
\begin{equation*}
    M \ge \Omega \Bigg ( \frac{ A\sigma^{2}}{mn\log m} \min \Bigg \{ \frac{1}{\min \{ B, 1\}}, \frac{mn}{\underset{i,j}{\max}n^{i}_{j}} \Bigg \} \Bigg )
\end{equation*}
\end{theorem}
\begin{proof}
Let us first introduce the following Lemma:
\begin{lemma}
\label{lemma:yuchenexpa}
Let V be sampled uniformly from $\{ -1,1\}^{d}$. For any $(i,j)$ assume that $X_{j}^{i}$ is independent of $\{ X_{j'}^{i}: j' \neq j\} \cup \{ V_{j'}: j^{'} \neq j \}$ given $V_{j}$. Let $P_{X_{j}}$ be the probability measure of $X_{j}$ and let $B_{j}^{i}$ be a set such that for some $\alpha^{i}_{j}$:
\begin{equation*}
    \sup_{S \in \sigma(B_{j}^{i})} \frac{P_{X_{j}}(S|V=v)}{P_{X_{j}}(S|V=v')} \le \exp(\alpha_{j}^{i})
\end{equation*}
Define random variable $E_{j}^{i} = 1$ f $X_{j}^{i} \in B_{j}^{i}$ and 0 otherwise. Then
\begin{equation*}
    I(V_{j},Y^{i}|V_{1:j-1}) \le H(E_{j}) + P(E_{j}=0) + 2(e^{4\alpha_{j}^{i}} - 1)^{2}I(X_{j}^{i}|V_{1:j-1})
\end{equation*}
Additionally if $\alpha_{j}^{i} < \frac{1.2564}{4}$, then the following is also true:
\begin{equation*}
    I(V_{j},Y^{i}|V_{1:j-1}) \le H(E_{j}) + P(E_{j}=0) + 128(\alpha_{j}^{i})^{2}I(X_{j}^{i}|V_{1:j-1})
\end{equation*}
\end{lemma}
\begin{proof}
The first statement is Lemma 4 of \cite{NIPS2013Yuchen}. \\The second statement directly follows from it, as for $x<1.2564$, it holds that $\exp(x) - 1 < 2x$
\end{proof}
Let us consider a problem where the reward for $j$th arm is sampled according to $X_{j} \sim \mathcal{N}(\delta V_{j},\sigma^{2})$, where $\delta$ is a parameter we will set later and $V_{j}$ is sampled uniformly from $\{-1,1\}$. Let us $V$ be a vector, whose $j$th element is $V_{j}$ and let $X_{j}^{i}$ be the samples from $j$th arm received by the $i$th centre. We will denote the number of samples from $j$th arm in the $i$th centre by $n_{j}^{i}$. Let $Y^{i}$ be the message send by the $i$th processing centre. We observe that $V \to X^{i} \to Y_{i}$ is a Markov Chain. We see that this scenario satisfies the assumptions required to use the method from Appendix \ref{appendix:minimaxlb}. Hence we would like to find a bound on $I(V,Y^{1:m})$ By tensorisation of information ((Lemma \ref{lemma:tenorisationinfo})) and the chain rule of information we get:
\begin{equation*}
    I(V,Y^{1:m}) \le \sum_{i=1}^{m}I(V,Y^{i}) = \sum_{i=1}^{m} \sum_{j=1}^{ A} I(V_{j},Y^{i}|V_{1:j-1})
\end{equation*}
If we define $B_{j}^{i} = \bigg \{ x \in \mathbb{R}^{n_{j}^{i}} : \big | \sum_{l=1}^{n_{j}^{i}} x_{l}\big | \le \sqrt{n_{j}^{i}a} \bigg \}$ for some $a$ then the condition from Lemma \ref{lemma:yuchenexpa} is satisfied by $\alpha_{j}^{i} = \frac{\sqrt{n_{j}^{i}}\delta a}{\sigma^{2}}$ and if we can set $a$ and $\delta$ such that $\alpha_{j}^{i} <\frac{1.2564}{4}$, then we have:
\begin{equation*}
    I(V,Y^{1:m}) \le \sum_{i=1}^{m} \sum_{j=1}^{ A} \bigg [ H(E_{j}^{i}) + P(E_{j}^{i}=0) + 128(\alpha_{j}^{i})^{2}I(X_{j}^{i}|V_{1:j-1}) \bigg ]
\end{equation*}
We will now bound each of the terms separately. Firstly as proven by \cite{NIPS2013Yuchen} (in proof of Lemma 5), we have:
\begin{equation*}
    P(E_{j}^{i}=0) \le 2 \exp \Bigg ( -\frac{\bigg ( a - \sqrt{n_{j}^{i}} \delta \bigg )^{2}}{2\sigma^{2}} \Bigg)
\end{equation*}
\begin{equation*}
    H(E_{j}^{i}) \le h \Bigg (2\exp \Bigg ( - \frac{ \big (a - \sqrt{n_{j}^{i}} \delta \big)^{2}}{2 \sigma^{2}} \Bigg ) \Bigg )
\end{equation*}
Now we focus on $I(X_{j}^{i}, Y|V_{1:j-1})$:
\begin{equation*}
I(X_{j}^{i}, Y^{i}|V_{1:j-1}) = H(Y^{i}|V_{1:j-1}) - H(Y^{i}|X_{j}^{i},V_{1:j-1}) \le H(Y^{i}|V_{1:j-1}) = 
\end{equation*}
\begin{equation*}
   = H(Y) - I(Y^{i},V_{1:j-1}) \le H(y) \le B
\end{equation*}
Hence we get that:
\begin{equation*}
    I(V, Y) \le\sum_{i=1}^{m} \sum_{j=1}^{ A} \Bigg [ 128\frac{n_{j}^{i}\delta^{2} a^{2}}{\sigma^{4}} B + h\bigg (2\exp \bigg ( - \frac{ \big (a - \sqrt{n_{j}^{i}} \delta \big)^{2}}{2 \sigma^{2}} \bigg ) \bigg ) + 2 \exp \Bigg ( -\frac{\big ( a - \sqrt{n_{j}^{i}} \delta \big )^{2}}{2\sigma^{2}} \Bigg) \Bigg]
\end{equation*}
Combining this with inequality \ref{eq:simple_info_bound}, we get:
\begin{equation*}
     I(V, Y) \le\sum_{i=1}^{m} \sum_{j=1}^{ A} \Bigg [ \frac{n_{j}^{i}\delta^{2} }{\sigma^{2}} \min \Big \{\frac{128Ba^{2}}{\sigma^{2}}, 1 \Big \}  + h\bigg (2\exp \bigg ( - \frac{ \big (a - \sqrt{n_{j}^{i}} \delta \big)^{2}}{2 \sigma^{2}} \bigg ) \bigg ) + 2 \exp \Bigg ( -\frac{\big ( a - \sqrt{n_{j}^{i}} \delta \big )^{2}}{2\sigma^{2}} \Bigg) \Bigg]
\end{equation*}
We now use the following notation for brevity:
\begin{equation*}
    A_{j}^{i} = \frac{n_{j}^{i}\delta^{2} }{\sigma^{2}} \min \Big \{\frac{128Ba^{2}}{\sigma^{2}}, 1 \Big \}
\end{equation*}
\begin{equation*}
    B_{j}^{i} = h\bigg (2\exp \bigg ( - \frac{ \big (a - \sqrt{n_{j}^{i}} \delta \big)^{2}}{2 \sigma^{2}} \bigg ) \bigg ) 
\end{equation*}
\begin{equation*}
    C_{j}^{i} =  2 \exp \Bigg ( -\frac{\big ( a - \sqrt{n_{j}^{i}} \delta \big )^{2}}{2\sigma^{2}} \Bigg)
\end{equation*}
We now set $a=5\sigma\sqrt{\log m}$ and we will now choose $\delta_{A}$, $\delta_{B}$ and $\delta_{C}$ for each term such that it is bounded and that $\delta_{B}$  satisfies the conditions of Lemma \ref{lemma:yuchenexpa}. Then we can just set $\delta = \min \{ \delta_{A}, \delta_{B}, \delta_{C} \}$. We do this for each term in turn:
\subsubsection*{$A$}
If we choose $\delta_{A}^{2}$ such that:
\begin{equation*}
    \delta_{A}^{2} \le \frac{\sigma^{2}}{10\sum_{i=1}^{m} \sum_{j=1}^{ A} n_{j}^{i} \min \Big \{\frac{128Ba^{2}}{\sigma^{2}}, 1 \Big \}} = \frac{\sigma^{2}}{10 \min \Big \{3200B\log m, 1 \Big \} \sum_{j=1}^{ A} \sum_{i=1}^{m} n_{j}^{i}}
\end{equation*}
Then we get the following bound:
\begin{equation*}
    \sum_{i=1}^{m} \sum_{j=1}^{ A} A_{j}^{i} = \delta^{2}\sum_{i=1}^{m} \sum_{j=1}^{ A} \frac{n_{j}^{i} \min \Big \{\frac{128Ba^{2}}{\sigma^{2}}, 1 \Big \}}{\sigma^{2}}  \le  \frac{1}{10}
\end{equation*}
\subsubsection*{$B$}
If we choose :
\begin{equation*}
    \delta^{2}_{B} \le \frac{\sigma^{2}}{400\log m \underset{i,j}{\max} n_{j}^{i}}
\end{equation*}
then we get that:
\begin{equation*}
    \alpha_{j}^{i} = \frac{\sqrt{n_{j}^{i}}\delta a}{\sigma^{2}} = \frac{\sqrt{n_{j}^{i}}}{4\sqrt{\underset{i,j}{\max} n_{j}^{i}}} \le \frac{1}{4} \le \frac{1.2564}{4}
\end{equation*}
which satisfies the second condition of Lemma \ref{lemma:yuchenexpa}. Also, we can see that $a > \sqrt{n_{j}^{i}} \delta $ and we get that $(a - \sqrt{n_{j}^{i}} \delta \big)^{2} \ge (5 - \frac{1}{20})^{2}\sigma^{2}\log m \ge 24 \sigma^{2} \log m$.
Since, for the binary entropy function we have $q(h) \le 6/5 \sqrt{q}$ for $q > 0$, we get that:
\begin{equation*}
     \sum_{i=1}^{m} \sum_{j=1}^{ A} B_{j}^{i} \le \sum_{i=1}^{m} \sum_{j=1}^{ A} h\bigg (2\exp \bigg ( - \frac{ \big (a - \sqrt{n_{j}^{i}} \delta \big)^{2}}{2 \sigma^{2}} \bigg ) \bigg ) \le \sum_{i=1}^{m} \sum_{j=1}^{ A} \frac{6\sqrt{2}}{5} \exp \bigg ( - \frac{24}{4}\log m \bigg ) < \frac{ A}{600}
\end{equation*}
\subsubsection*{$C$}
If we bound $\delta_{C}$ in the same way as $\delta_{B}$, we get that:
\begin{equation*}
     \sum_{i=1}^{m} \sum_{j=1}^{ A} C_{j}^{i} \le \sum_{i=1}^{m} \sum_{j=1}^{ A} 2 \exp \Bigg ( -\frac{\big ( a - \sqrt{n_{j}^{i}} \delta \big )^{2}}{2\sigma^{2}} \Bigg) \le 2 dm \exp (-12\log m) = \frac{2d}{m^{11}} \le \frac{ A}{10^{6}}
\end{equation*}
Hence we now have a $\delta$ and we can construct the lower bound as described in Appendix \ref{appendix:minimaxlb}. We get that for $d > 12$:
\begin{equation*}
    M(\theta, P, B) \ge \delta^{2} \Big (\floor{\frac{ A}{6}} + 1 \Big ) \Bigg ( 1 - \frac{I(Y,V) + \log2}{\frac{ A}{6}} \Bigg ) \ge \delta^{2} \Big (\floor{\frac{ A}{6}} + 1 \Big ) \Bigg ( 1 - \frac{\frac{1}{10} + \frac{ A}{600} +  \frac{ A}{10^{6}} + \log2}{\frac{ A}{6}} \Bigg )
\end{equation*}
\begin{equation*}
    \ge \delta^{2} \Big (\floor{\frac{ A}{6}} + 1 \Big ) \Bigg ( 1 - \frac{10^{6} + 600}{10^{8}} - \frac{\frac{1}{10} + \log2}{\frac{ A}{6}} \Bigg )
\end{equation*}
Since for $ A>12$, the expression in second brackets is always positive, we have that $M(\theta, P, B) \ge \Omega(\delta^{2} A)$. Substituting $\delta = \min \{\delta_{A}, \delta_{B}, \delta_{C} \}$ gives:

\begin{equation*}
    M \ge \Omega \Bigg ( \frac{ A\sigma^{2}}{\log m} \min \Bigg \{ \frac{1}{\min \Big \{B\log m, 1 \Big \} \sum_{j=1}^{ A} \sum_{i=1}^{m} n_{j}^{i}}, \frac{1}{\underset{i,j}{\max}n^{i}_{j}} \Bigg \} \Bigg )
\end{equation*}
We see that: 
\begin{equation*}
    \sum_{j=1}^{ A}  \sum_{i=1}^{m} n^{i}_{j} = mn
\end{equation*}
which completes the proof.
\end{proof}


\subsection{Results for Off-policy Linear Value Function Approximation}
\begin{assumption} \label{as:boundedISratio}
For any $s \in S$, we have that $\textrm{supp}(\pi_{t}(a|s)) \subset \textrm{supp}(\pi_{b}(a|s))$ and $ \frac{\pi_{t}(a|s)}{\pi_{b}(a|s)} \le \rho_{\textrm{max}}$.
\end{assumption}
We present the following lower bound:
\begin{theorem} \label{th:offpolicyvfalb}
In a distributed off-policy linear value funcion approximation problem with context dimensionality of $ C>12$ and state space size of $ S>1$, under assumptions \ref{as:boundedparam}, \ref{as:boundedeigen}, \ref{as:boundedreturn}, \ref{as:episodesforstate} and \ref{as:boundedISratio}, given $m$ processing centres each with $E$ episodes for each state, with each centre having a communication budget $B \ge 1$, the minimax risk $M$ of any algorithm is lower bounded as:
\begin{equation*}
    M \ge \Omega \Bigg ( \frac{ C\rho_{\textrm{max}}^2G_{\textrm{max}}^{2}}{SEm\lambda_{\textrm{max}}} \min \Bigg \{ \frac{SEm\lambda_{\textrm{max}}}{\rho_{\textrm{max}}^2G_{\textrm{max}}^{2}} ,\frac{1}{ \min\big\{\frac{B}{ C}, 1 \big \}\log m}, \frac{m}{\log m} \Bigg \} \Bigg )
\end{equation*}
\end{theorem}
\begin{proof}
We consider a MDP with $ S$ states, where at each state agent takes one of two actions. Selecting action $a=2$ gives a reward of 0 always and selecting action $a=1$ gives a reward sampled from a distribution with mean of $\mu_{i}$ for state $i$. We consider the following behaviour and target policies:
\begin{equation*}
    \pi_{t} = \begin{cases}
    \frac{1}{\rho_{\textrm{max}} + 1} \textrm{ for } a = 1 \\
    1 - \frac{1}{\rho_{\textrm{max}} + 1} \textrm{ for } a = 2
    \end{cases}
\end{equation*}
\begin{equation*}
    \pi_{b} = \begin{cases}
    1 - \frac{1}{\rho_{\textrm{max}} + 1} \textrm{ for } a = 1 \\
    \frac{1}{\rho_{\textrm{max}}+ 1} \textrm{ for } a = 2
    \end{cases}
\end{equation*}
We see that in this construction, the ratios of probabilities of choosing each action under both policies are always bounded by $\rho_{\textrm{max}}$. The value function of target policy under such construction for each state is thus $v(i) = \vc_{i}^T\theta = \frac{\mu}{\rho_{\textrm{max}} + 1}$, so the mean reward for action $a=1$ can be expressed as $\mu = (\rho_{\textrm{max}} + 1)\vc_{i}^T\theta$. We can thus follow a similar idea as in the proof of Theorem \ref{th:lvfmdp} and set $r_{i,k} = (2p_{i,k} - 1)G_{\textrm{max}}$ where $p_{i,k} \sim \textrm{Bernoulli}(\frac{1}{2} + \frac{c_{i,k}v_{k}\delta}{2G_{\textrm{max}}(\rho_{\textrm{max}} + 1)})$. Proceeding mutatis mutandis  completes the proof.
\end{proof}
%What is Rao-Cramer for importance sampling? Weighted Importance Sampling?

